Learning From Graph-Structured Data: Addressing Design Issues and Exploring Practical Applications in Graph Representation Learning

Graphs serve as fundamental descriptors for systems composed of interacting elements, capturing a wide array of data types, from molecular interactions to social networks and knowledge graphs. In this paper, we present an exhaustive review of the latest advancements in graph representation learning and Graph Neural Networks (GNNs). GNNs, tailored to handle graph-structured data, excel in deriving insights and predictions from intricate relational information, making them invaluable for tasks involving such data. Graph representation learning, a pivotal approach in analyzing graph-structured data, facilitates numerous downstream tasks and applications across machine learning, data mining, biomedicine, and healthcare. Our work delves into the capabilities of GNNs, examining their foundational designs and their application in addressing real-world challenges. We introduce a GNN equipped with an advanced high-order pooling function, adept at capturing complex node interactions within graph-structured data. This pooling function significantly enhances the GNN's efficacy in both node- and graph-level tasks. Additionally, we propose a molecular graph generative model with a GNN as its core framework. This GNN backbone is proficient in learning invariant and equivariant molecular characteristics. Employing these features, the molecular graph generative model is capable of simultaneously learning and generating molecular graphs with atom-bond structures and precise atom positions. Our models undergo thorough experimental evaluations and comparisons with established methods, showcasing their superior performance in addressing diverse real-world challenges with various datasets.

==> Chapters/Findings.tex <==
\chapter{Discussion of Findings}
In this work, we study the capabilities of Graph Neural Networks (GNNs),  exploring their fundamental designs and applications to address real-world challenges. In particular, introduce a GNN featuring a high-order pooling function, capturing complex interactions between nodes in graph-structured data. designed to capture intricate interactions between nodes in graph-structured data. This pooling function enhances the GNN's performance on both node- and graph-level tasks. Furthermore, we propose a GNN as the backbone model for a molecular graph generative model. The GNN backbone is adept at learning both the invariant and the equivariant aspects of molecules. The molecular graph generative model leverages these features to simultaneously learn and generate atom-bond molecular graphs with atom positions. Our models are rigorously evaluated through experiments and comparisons with existing methods, demonstrating their effectiveness in tackling real-world problems with diverse datasets.

\section{Understanding of High-Order Pooling}
In our discussion, we emphasize the significance of high-order pooling among node features in graphs. This concept pertains to the multi-dimensional interactions between nodes within their neighborhood.

We introduce a tensorized-GNN equipped with a high-order pooling function, designed to model these complex, multi-dimensional node feature interactions. For instance, given node features $x_1, x_2, x_3$, a conventional linear sum pooling in a GNN layer would yield a vector like $[x_1 + x_2 + x_3]$. In contrast, our high-order layer, inspired by tensor products, generates a vector $[x_1, x_2, x_3, x_1 + x_2, x_1 + x_3, x_2 + x_3, x_1 + x_2 + x_3, x_1x_2, x_1x_3, x_2x_3, x_1x_2x_3]$ with 11 terms. This approach is considerably more expressive than the linear sum pooling commonly used in GNNs. In traditional GNN contexts, "high-order" typically refers to capturing long-range node dependencies \cite{xu2018powerful, baek2021accurate, wang2020second}, but our approach is unique in focusing on multi-dimensional feature products. Yet, like other GNNs \cite{kipf2016classification, velivckovic2017attention}, our model can also capture long-range dependencies by stacking layers.

The rationale behind computing multi-dimensional feature products becomes clear when considering multi-dimensional feature spaces. Taking a molecular graph dataset as an example, consider blood pressure as one feature. Many studies have examined blood pressure's impact on health. To predict life expectancy, one might initially consider using just blood pressure. However, this single feature is often insufficient. Adding other features like age, exercise frequency, and body fat creates a multi-dimensional feature vector for each individual. A simple GNN, using linear feature interactions, may not capture the correlations among age, exercise frequency, and body fat. These correlations are crucial for predicting life expectancy. Our model, with its multi-dimensional feature products, can capture interactions like age$\times$exercise frequency, age$\times$body fat, exercise frequency$\times$body fat, and age$\times$exercise frequency$\times$body fat, which are vital for accurate predictions. This concept is particularly relevant in molecular graphs, where features such as atomic charge and mass are often correlated. The importance of high-dimensional feature products extends to other networks and applications as well \cite{novikov2016exponential, stoudenmire1605supervised}.

Therefore, we confidently assert that our tensorized-GNN with its high-order pooling function plays a crucial role in learning interactions between nodes within a neighborhood. By computing more expressive products between node features, this approach enhances the representation of node interactions. Furthermore, it offers an innovative method for computing non-linear interactions between node features through tensor decomposition, providing a significant advancement in graph neural network capabilities.


\section{Importance of Co-Generation}
GNNs can be used as the backbone model of generative models for molecules for learning their hidden representations. We propose a graph transformer, namely MUformer, to learn the hidden representations of molecular structures (bonds and edges) and their atom arrangements (atom coordinates). And the backbone model allows the co-generation of both molecular structures and their geometry in our generative diffusion model. Here, we discuss the importance of co-generation of molecular structures and geometry in a generative process.

Co-generation of molecular structures and geometry is important for several reasons. First, it enables the generation of novel molecules that are not only chemically valid, but also physically realistic. By jointly modeling the 2D topology and 3D geometry of molecules, the generative model can capture the complex interactions and constraints between atoms and bonds, and avoid producing unrealistic or unstable structures. Second, it facilitates the optimization of molecular properties and functionalities that depend on both the structure and the geometry of molecules. For example, the binding affinity of a drug molecule to a target protein is largely determined by the shape and orientation of the molecule, as well as its chemical composition. By co-generating the molecular structure and geometry, the generative model can explore the trade-offs and synergies between different aspects of molecular design, and generate molecules that satisfy multiple objectives. Third, it enriches the representation and diversity of the generated molecules, and expands the search space of the generative model. By incorporating 3D geometric information into the molecular graph generation, the generative model can learn more expressive and informative features of molecules, and generate more diverse and novel molecular graphs. Conversely, by using the molecular graph information to guide the prediction of molecular geometry, the generative model can generate more accurate and consistent molecular structures.

In summary, co-generation of molecular structures and geometry is a promising direction for machine learning-based molecule design, as it can improve the validity, realism, functionality, and diversity of the generated molecules. Our proposed framework, MUDiff, is a roto-translation equivariant generative model that can effectively co-generate molecular graphs and structures, and outperform previous methods on various tasks. We hope that our work can inspire more research on the integration of 2D topology and 3D geometry in molecule generation, and provide new insights into the structure-property relationship of molecules.


\section{Limitations of Pooling Function}
In this thesis, we have presented a novel approach for high-order pooling for graph neural networks, based on symmetric tensor decomposition. Our approach, tGNN, can model non-linear high-order multiplicative interactions among node representations, and achieve state-of-the-art performance on various graph classification tasks. However, there are still some limitations and challenges that can be addressed in future work.

One limitation of our approach is that it requires a fixed number of node representations to be aggregated by the CP layer, which may not be suitable for graphs with varying sizes or structures. Therefore, a possible direction for future work is to explore how to adapt the CP layer to handle variable-sized inputs, such as using attention mechanisms, dynamic programming, or graph coarsening techniques.

Another challenge of our approach is that it relies on a predefined set of basis tensors to parameterize the CP layer, which may limit the expressiveness and flexibility of the model. Moreover, the choice of the basis tensors may affect the computational efficiency and stability of the model. Therefore, another direction for future work is to develop more adaptive and efficient methods to learn the basis tensors from the data, such as using neural networks, sparse coding, or tensor factorization methods.

A third challenge of our approach is that it does not explicitly incorporate edge features or edge weights into the aggregation function, which may ignore some important information or relationships in the graph. Therefore, a third direction for future work is to explore how to extend the CP layer to account for edge features or edge weights.



\section{Limitations of Generative Model}
In this thesis, we have presented a novel framework for co-generating molecular structures and geometry, based on a graph transformer backbone and a generative diffusion model. Our framework, MUDiff, can generate realistic and diverse molecules that satisfy various design objectives and constraints. However, there are still some limitations and challenges that need to be addressed.

One limitation of our framework is that it requires a large and high-quality dataset of molecular graphs and structures to train the model. However, such datasets are not always available or easy to obtain, especially for specific domains or applications. Therefore, a possible direction for future work is to explore how to leverage other sources of data, such as synthetic or simulated data, to augment the training data and improve the model performance.

Another challenge of our framework is that it relies on a fixed and predefined set of atom types and bond types, which may limit the diversity and novelty of the generated molecules. Moreover, the model may not be able to handle new or rare atom types or bond types that are not seen in the training data. Therefore, another direction for future work is to develop more flexible and adaptive methods to represent and generate molecular graphs and structures, such as using continuous or latent variables to encode the atom types and bond types, or using graph neural networks to learn the atom types and bond types from the data.



==> Chapters/GNN.vs.MLP..tex <==
\chapter{Graph Neural Networks Meet Heterophilic Datasets}
In this chapter, we explore the limitations of employing Graph Neural Networks (GNNs), particularly in comparison to traditional NNs for node-level classification in heterophilic graph datasets. We highlight the underperformance of GNNs in such scenarios.
Our analysis reveals shortcomings in current metrics designed to measure homophily/heterophily levels, prompting the proposal of a more effective metric grounded in graph structure, label consistency, and post-aggregation information. We lao introduce a universal GNN framework adaptable to various GNN designs. This framework is designed to dynamically learn representations for both homophilic and heterophilic graph datasets.

\section{Preliminaries}

\section{Underperformance of GNNs on Heterohphilic Datasets}
\input{Tables1/gnn.vs.mlp.tex}
In Tab.~\ref{tab:gnn.vs.mlp}, we discover that several GNN baselines, e.g., GCN \cite{kipf2016classification}, GAT \cite{velivckovic2017attention}, and GraphSAGE \cite{hamilton2017inductive}, fail to outperform MLPs on node-level classification for several graphs. 
This demonstrates that GNNs do not always gain advantages over traditional NNs when dealing with relational data. 
This underperformance of GNNs have been explained by the low homophily (or heteorphily) issue of these graph structures \cite{luan2020complete, zhu2020beyond, luan2022we}.
Homophily describes nodes from  the same category are more likely to be connected, which is believed to be the key of the success for GNNs. 
Heterophily, on the other hand, describes a scenario where nodes from different categories are more likely to be connected, and causes nodes to be indistinguishable to GNNs \cite{zhu2020beyond, luan2021heterophily}. 

\subsection{Metrics of Homophily}
People propose metrics to measure the level of homophily for graphs. These metrics of homophily are defined by considering different relations between node labels and graph structures defined by adjacency matrix,
\begin{equation}
\begin{aligned}
\label{eq:definition.homophily.metrics}
    &H_\text{edge}(\mathcal{G}) = \frac{\big|\{e_{uv} \mid e_{uv}\in \mathcal{E}, Z_{u,:}=Z_{v,:}\}\big|}{|\mathcal{E}|}, \\ 
    &H_\text{node}(\mathcal{G}) = \frac{1}{|\mathcal{V}|} \sum_{v \in \mathcal{V}} 
    \frac{\big|\{u \mid u \in \mathcal{N}_v, Z_{u,:}=Z_{v,:}\}\big|}{d_v}, \\
    &H_\text{class}(\mathcal{G}) = \frac{1}{C-1} \sum_{k=1}^{C}\left[h_{k}
    -\frac{\big|\{v \mid Z_{v,k} = 1 \}\big|}{N}\right]_{+}, \ \ 
    h_{k}=\frac{\sum_{v \in \mathcal{V}} \big|\{u \mid Z_{v,k} = 1, u \in \mathcal{N}_v,   Z_{u,:}=Z_{v,:}\}\big| }{\sum_{v \in \{v|Z_{v,k}=1\}} d_{v}},
\end{aligned}
\end{equation}
where $H_\text{edge}(\mathcal{G})$ measures the edge homophily \cite{abu2019mixhop,zhu2020beyond}, $H_\text{node}(\mathcal{G})$ measures the node homophily \cite{pei2020geom}, $H_\text{class}(\mathcal{G})$ measures the class homophily \cite{lim2021new}, and $[\cdot]_+ = \max (0, \cdot)$. They all lie in the range of $[0, 1]$ and a value close to $1$ corresponds to strong homophily while a value close to $0$ indicates strong heterophily. 
$H_\text{edge}(\mathcal{G})$ measures the proportion of edges that connect two nodes in the same class; $H_\text{node}(\mathcal{G})$ evaluates the average proportion of edge-label consistency of all nodes; $H_\text{class}(\mathcal{G})$ tries to avoid the sensitivity to imbalanced class, which can cause $H_\text{edge}$ misleadingly large. 
The above definitions are all based on the graph-label consistency and imply that the inconsistency will cause harmful effect to the performance of GNNs. 
With this in mind, we will show a counter example to illustrate the insufficiency of the above metrics and propose new metrics in the following section.

\begin{figure}[htbp!]
    \centering
     {
     {
    \subfloat[ \texttt{Cornell}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_cornell.pdf}
     } 
     \subfloat[ \texttt{Wisconsin}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_wisconsin.pdf}
     } 
     \subfloat[ \texttt{Texas}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_texas.pdf}
     } \\
     \subfloat[ \texttt{Chameleon}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_chameleon.pdf}
     } 
     \subfloat[ \texttt{Squirrel}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_squirrel.pdf}
     } 
     \subfloat[ \texttt{Film}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_film.pdf}
     } \\
     \subfloat[ \texttt{Cora}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_cora.pdf}
     } 
     \subfloat[ \texttt{Citeseer}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_citeseer.pdf}
     } 
     \subfloat[ \texttt{Pubmed}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.33\textwidth]{Images1/local_homo_pubmed.pdf}
     } 
     }
     }
     \caption{$H_\text{node}^v$ distributions of different datasets}
     \label{fig:local_homo_distributions}
\end{figure}
\subsection{Node Local Homophily Distributions of Real-World Datasets}
In Fig.~\ref{fig:local_homo_distributions}, we show the distributions of node homophily $H_\text{node}^v$ for 9 grap datasets.
We can see that \textit{Wisconsin} and \textit{Texas} have high density in low homophily area, \textit{Cornell, Chameleon, Squirrel} and \textit{Film} have high density in low and middle homophily area, \textit{Cora, CiteSeer} and \textit{PubMed} have high density in high homophily area.

\section{Analysis of Heterophily}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\textwidth]{Images1/fig.bipartite.pdf}
    \caption{Example of harmless heterophily}
  \label{fig:example.harmless.heterophily}
\end{figure}
Heterophily is believed to be harmful for message-passing based GNNs \cite{zhu2020beyond, pei2020geom} because intuitively features of nodes in different classes will be falsely mixed and this will lead nodes indistinguishable.
However, it is not always the case \cite{luan2022revisiting, luan2023graph}, e.g., the bipartite graph shown in Fig.~\ref{fig:example.harmless.heterophily} is highly heterophilic according to the existing homophily metrics in Eq.~\ref{eq:definition.homophily.metrics}, but nodes are still distinguishable after the aggregation because the nodes from two classes just exchange colors. This example encourages us to study the relation between nodes after the aggregation.
Therefore, we first define the post-aggregation node similarity matrix as follows:
\begin{equation}
\label{eq:post.agg.similarity.matrix}
    S(\hat{A},X) \equiv \hat{A}X (\hat{A}X)^T \in \mathbb{R}^{N\times N},
\end{equation}
where $\hat{A} \in \mathbb{R}^{N\times N}$ denotes a general aggregation operator. $S(\hat{A},X)$ is essentially the gram matrix that measures the similarity between each pair of aggregated node features.


\subsection{Aggregation Similarity Score}
A generalized GNN output can be expressed as:
\begin{equation}
    \begin{aligned}
    Y  = \text{Softmax} (\hat{A}  X W ) = \text{Softmax} (Y').
    \end{aligned}
\end{equation}
With the loss function of a GNN, $\mathcal{L}  = -\text{trace}(Z^T \log Y)$, we have $\Delta W = \gamma \frac{d \mathcal{L}}{d W}$ after each gradient descent step, where $\gamma$ is the learning rate.
The update of $Y'$ is analyzed in \cite{luan2022revisiting} as:
\begin{equation}
    \begin{aligned}
    \label{eq:gradient.descent.update}
    \Delta Y' & = \hat{A} X \Delta W = \gamma \hat{A}X \frac{d \mathcal{L}}{d W} \propto \hat{A}X \frac{d \mathcal{L}}{d W} = \hat{A}X X^T\hat{A}^T (Z-Y) = S(\hat{A},X) (Z-Y),
    \end{aligned}
\end{equation}
where $Z-Y$ is the prediction error matrix. The update direction of the prediction for node $i$ is essentially a weighted sum of the prediction error, i.e., $\Delta (Y')_{i,:} = \sum_{j\in \mathcal{V}} \big[S(\hat{A},X)\big]_{i,j} (Z-Y)_{j,:}$ and $\big[S(\hat{A},X)\big]_{i,j}$ can be considered as the weights. Intuitively, a high similarity value $\big[S(\hat{A},X)\big]_{i,j}$ means node $i$ tends to be updated to the same class as node $j$. This indicates that $S(\hat{A},X)$ is closely related to a single layer GNN model.

Based on the above definition and observation, we define the aggregation similarity score as follows.
\begin{definition} The aggregation similarity score is: %based on $S(\hat{A},X)$
\begin{equation}
\begin{aligned}
\label{eq:aggregation.similarity}
     S_\text{agg}\big(S(\hat{A},X)\big) 
    = \frac{1}{\left| \mathcal{V} \right|} \left| \left\{v   \,\big| \,
    \mathrm{Mean}_u\big( \{S(\hat{A},X)_{v,u} | Z_{u,:}=Z_{v,:} \}\big) 
    \geq  \mathrm{Mean}_u\big(\{S(\hat{A},X)_{v,u} | Z_{u,:} \neq Z_{v,:} \} \big) \right\} \right|,
\end{aligned}
\end{equation}
where $\mathrm{Mean}_u\left(\{\cdot\}\right)$ takes the average over $u$ of a given multiset of values or variables.
\end{definition}
$S_\text{agg}(S(\hat{A},X))$ measures the proportion of nodes $v\in\mathcal{V}$ as which the average weights on the set of nodes in the same class (including $v$) is larger than that 
in other classes. In practice, we rescale Eq.~\eqref{eq:aggregation.similarity} to the following modified aggregation similarity,
\begin{equation}
\label{eq:modified.aggregation.homophily}
  S^M_\text{agg}\big(S(\hat{A},X)\big) = \big[2 S_\text{agg}\big(S(\hat{A},X)\big)-1\big]_{+} \in [0, 1].
\end{equation}
Based on the analysis of post-aggregation node similarity matrix and aggregation similarity score, we propose the graph aggregation homophily metric to better measure the homophily level based on the graph structure and label consistency.


\subsection{Graph Aggregation Homophily}
In order to measure the consistency between labels and graph structures without considering node features and to make a fair comparison with the existing homophily metrics in Eq.~\ref{eq:definition.homophily.metrics}, we define the graph ($\mathcal{G}$) aggregation ($\hat{A}$) homophily and its modified version \footnote{In practice, we will only check $H_{\text{agg}}(\mathcal{G})$ when $H_{\text{agg}}^M(\mathcal{G})=0$.} as:
\begin{equation}
    \label{eq:aggregation.homophily.metrics}
    H_{\text{agg}}(\mathcal{G}) = S_\text{agg}\big(S(\hat{A},Z)\big)\!, \; H_{\text{agg}}^M(\mathcal{G}) = S_\text{agg}^M\big(S(\hat{A},Z)\big).
\end{equation}
As the example shown in Fig.~\ref{fig:example.harmless.heterophily}, when $\hat{A} = \hat{A}_\text{rw}$, it is easy to see that $H_{\text{agg}}(\mathcal{G}) = H_{\text{agg}}^M(\mathcal{G}) = 1$ and other metrics are 0. Thus, this new metric reflects the fact that nodes from two classes are still highly distinguishable after aggregation, while other metrics mentioned before fail to capture such information and misleadingly give value 0. This shows the advantage of $H_{\text{agg}}(\mathcal{G})$ and $H_{\text{agg}}^M(\mathcal{G})$, which additionally exploit information from aggregation operator $\hat{A}$ and the similarity matrix.

\subsection{Evaluation on Synthetic Graphs}
We conduct experiments on synthetic graphs generated with different levels of $H_{\text{edge}}^M(\mathcal{G})$ to assess the output of $H_{\text{agg}}^M(\mathcal{G})$ in comparison with existing metrics.
\begin{figure}[htbp]
\centering
 {
    {
     \subfloat[$H_\text{edge}(\mathcal{G})$]{
     \captionsetup{justification = centering}
     \includegraphics[height=0.1\textheight]{Images1/fig_Edge_Homophily_comparison.pdf}
     } 
     \subfloat[$H_\text{node}(\mathcal{G})$]{
     \captionsetup{justification = centering}
     \includegraphics[height=0.1\textheight]{Images1/fig_Node_Homophily_comparison.pdf}
     }
     \subfloat[$H_\text{class}(\mathcal{G})$]{
     \captionsetup{justification=centering}
     \includegraphics[height=0.1\textheight]{Images1/fig_Class_Homophily_comparison.pdf}
     } 
     \subfloat[$H_{\text{agg}}^M(\mathcal{G})$]{
     \captionsetup{labelsep=newline,format=plain,indention=-100pt}
     \includegraphics[height=0.1015\textheight]{Images1/fig_Modified_Agg_Homophily_comparison_legend2.pdf}
     }
     }
     }
     \caption{Comparison of baseline performance under different homophily metrics.}
     \label{fig:comparison.homophily.metrics}
\end{figure}

We first generated 10 graphs for each of 28 edge homophily levels, from 0.005 to 0.95, for a total of $280$ graphs. 
In every generated graph, we had 5 classes, with 400 nodes in each class. For nodes in each class, we randomly generated 800 intra-class edges and [$\frac{800}{H_\text{edge}(\mathcal{G})} -800$] inter-class edges. 
The features of nodes in each class are sampled from node features in the corresponding class of $6$ base datasets (\textit{Cora, CiteSeer, PubMed, Chameleon, Squirrel, Film}). 
Nodes were randomly split into  train/validation/test sets, in proportion of 60\%/20\%/20\%. 
We trained 1-hop SGC (\textit{sgc-1}) \cite{wu2019simplifying} and GCN \cite{kipf2016classification} on the synthetic graphs.
For each value of $H_\text{edge}(\mathcal{G})$, we take the average test accuracy and standard deviation of runs over the 10 generated graphs with that value. For each generated graph, we also calculate $H_{\text{node}}(\mathcal{G}), H_{\text{class}}(\mathcal{G})$ and $H_{\text{agg}}^M(\mathcal{G})$. 
Model performance with respect to different homophily values is shown in Fig.~\ref{fig:comparison.homophily.metrics}.

The performance of SGC-1 and GCN is expected to be monotonically increasing if the homophily metric is informative. However, Fig.~\ref{fig:comparison.homophily.metrics}(a)(b)(c) show that the performance curves under $H_{\text{edge}}(\mathcal{G}), H_{\text{node}}(\mathcal{G})$ and $H_{\text{class}}(\mathcal{G})$ are $U$-shaped, while Fig.~\ref{fig:comparison.homophily.metrics}(d) reveals a nearly monotonic curve with a little numerical perturbation around 1. 
This indicates that $H_{\text{agg}}^M(\mathcal{G})$ provides a better indication of the way in which the graph structure affects the performance of SGC-1 and GCN than existing metrics. 
After proposing a concrete metric to better measure the homophily level of a graph, we aim to address the underperformance issue of GNNs cased by heterophily.

\section{High-Pass Filter and Heterophily}
In prior work~\cite{luan2020complete,bo2021beyond}, it has been shown that high-frequency graph signals, which can be extracted by a high-pass filter, i.e., diversification operation, is empirically useful for addressing heterophily. Here, we give thorough analysis based on the similarity matrix in Eq.~\ref{eq:gradient.descent.update}. 
\begin{figure}[htbp!]
  \begin{center}
    \includegraphics[width=.8\textwidth]{Images1/fig_HP_successful_example.pdf}
  \end{center}
  \caption{Example of how diversification can address harmful heterophily}
  \label{fig:successful_example_hp_filter}
\end{figure}
We first consider the example shown in Figure \ref{fig:successful_example_hp_filter}. 
From $S(\hat{A},X)$, we can see that nodes $\{1,3\}$ assign relatively large positive weights to nodes in class 2 after aggregation, which will %cause harmful effect for learning
make nodes $\{1,3\}$ hard to be distinguished from nodes in class 2. However, we can still %tell the difference
distinguish nodes $\{1,3\}$ and $\{4,5,6,7\}$ by considering % into account their neighborhood differences
their neighborhood differences: nodes $\{1,3\}$ are different from most of their neighbors while nodes $\{4,5,6,7\}$ are similar to most of their neighbors. This indicates that although some nodes become similar after aggregation, they are still distinguishable through their local surrounding dissimilarities. 

This observation leads us to introduce the \textit{diversification operation}, i.e., HP filter $I-\hat{A}$ \cite{ekambaram2014graph} to extract information regarding neighborhood differences, thereby addressing harmful heterophily. As $S(I-\hat{A},X)$ in Fig.~\ref{fig:successful_example_hp_filter} shows, nodes $\{1,3\}$ will assign negative weights to nodes $\{4,5,6,7\}$ after the diversification operation,i.e., nodes $1,3$ treat nodes $4,5,6,7$ as negative samples and will move away from them during backpropagation. This example reveals that there are cases in which the diversification operation is helpful to handle heterophily, while the aggregation operation is not. Thus, we introduce the concept of filterbank which combines both LP (aggregation) and HP (diversification) filters and can potentially handle various local heterophily cases.

\subsection{Filterbank}
For the graph signal $\mathbf{x}$ defined on $\mathcal{G}$, a 2-channel linear (analysis) filterbank \cite{ekambaram2014graph} \footnote{In graph signal processing, an additional synthesis filter \cite{ekambaram2014graph} is required to form the 2-channel filterbank. But a synthesis filter is not needed in our framework.} includes a pair of  filters $H_\text{LP}, H_\text{HP}$, which retain the low-frequency and high-frequency content of $\mathbf{x}$, respectively.
Most existing GNNs use a uni-channel filtering architecture \cite{kipf2016classification,velivckovic2017attention,hamilton2017inductive} with either LP or HP channel, which only partially preserves the input information. Unlike the uni-channel architecture, filterbanks with $H_\text{LP} + H_\text{HP} = I$ do not lose any information from the input signal, which is called the perfect reconstruction property \cite{ekambaram2014graph}. Generally, the Laplacian matrices ($L_\text{sym}$, $L_\text{rw}$, $\hat{L}_\text{sym}$, $\hat{L}_\text{rw}$) can be regarded as HP filters \cite{ekambaram2014graph} and affinity matrices ($A_\text{sym}$, $A_\text{rw}$, $\hat{A}_\text{sym}$, $\hat{A}_\text{rw}$) can be treated as LP filters \cite{maehara2019revisiting, hamilton2020graph}. Moreover,  we extend the concept of filterbank and view MLPs as using the identity (full-pass) filterbank with $H_\text{LP}=I$ and $H_\text{HP}=0$, which also satisfies $H_\text{LP} + H_\text{HP} = I+0 = I$.

\subsection{Node-wise Channel Mixing}
The example in  Fig.~\ref{fig:successful_example_hp_filter} also shows that different nodes may need the local information extracted from different channels, i.e., nodes $\{1,3\}$ demand information from the HP channel while node 2 only needs information from the LP channel.
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=.4\textwidth]{Images1/local_homo_4.pdf}
  \end{center}
  \caption{$H_\text{node}^v$ distributions}
  \label{fig:local_homophily_4}
\end{figure}
Fig.~\ref{fig:local_homophily_4} reveals that nodes have diverse distributions of node local homophily $H_\text{node}^v$ across different datasets. In order to adaptively leverage the LP, HP and identity channels in GNNs to deal with the diverse local heterophily situations, we introduce our proposed Adaptive Channel Mixing (ACM) framework.

\section{Adacptive Channel Mixing for GNNs}
\label{sec:filterbank_acm_gnn_architecture}
We will use GCN as an example to introduce the ACM framework in matrix form, but the framework can be combined in a similar manner to many different GNNs.
%We use $H_\text{LP}$ and $H_\text{HP}$ to represent general LP and HP filters.
The ACM framework includes the following steps:
\begin{equation*}
\begin{aligned}
\label{eq:acm_gnn_spectral}
& \textbf{{Step 1. Feature Extraction for Each Channel:}} \\
& \resizebox{1\hsize}{!}{$\text{Option 1: } {H}^{l}_L = \text{ReLU}\left(H_\text{LP} {H^{l-1}} W^{l-1}_L\right), {{H}^{l}_H} =  \text{ReLU}\left(H_\text{HP} {H^{l-1}} W^{l-1}_H\right), {H}^{l}_I  = \ \text{ReLU}\left(I {H^{l-1}} W^{l-1}_I\right);$} \\
& \resizebox{1\hsize}{!}{$ \text{Option 2: } {H}^{l}_L = H_\text{LP} \text{ReLU}\left({H^{l-1}} W^{l-1}_L\right), {{H}^{l}_H} = H_\text{HP} \text{ReLU}\left({H^{l-1}} W^{l-1}_H\right), {H}^{l}_I  = I\ \text{ReLU}\left({H^{l-1}} W^{l-1}_I\right); $} \\
& H^0=X \in \mathbb{R}^{N\times F_0}, \ W_L^{l-1},\ W_H^{l-1}, \ W_I^{l-1} \in \mathbb{R}^{F_{l-1} \times F_l},\ l = 1,\dots,L;\\
& \textbf{Step 2. Row-wise Feature-based Weight Learning:} \\
&\resizebox{1\hsize}{!}{$ \tilde{\alpha}_L^l = \text{Sigmoid} \left({H}^{l}_L \tilde{W}^{l}_L\right),\ \tilde{\alpha}_H^l = \text{Sigmoid} \left({H}^{l}_H \tilde{W}^{l}_H\right), \tilde{\alpha}_I^l = \text{Sigmoid} \left({H}^{l}_I \tilde{W}^{l}_I\right),\ \tilde{W}_L^{l-1},\ \tilde{W}_H^{l-1},\ \tilde{W}_I^{l-1} \in \mathbb{R}^{F_l \times 1} $} \\ 
& \left[{\alpha}_L^l, {\alpha}_H^l, {\alpha}_I^l \right] = \text{Softmax}\left((\left[\tilde{\alpha}_L^l,\tilde{\alpha}_H^l,\tilde{\alpha}_I^l\right]/T) W_\text{Mix}^l \right) \in \mathbb{R}^{N\times 3}, T \in \mathbb{R} \text{ temperature},\ W_\text{Mix}^l \in \mathbb{R}^{3\times 3}; \\
&\textbf{Step 3. Node-wise Adaptive Channel Mixing:}&\\
&{H^{l}}  =  \text{ReLU}\left(\text{diag}(\alpha_L^l){H}^{l}_L + \text{diag}(\alpha_H^l){H}^{l}_H + \text{diag}(\alpha_I^l){H}^{l}_I \right)&
\end{aligned}
\end{equation*}
We will refer to the instantiation which uses option 1 in step 1 as ACM and to the one using option 2 as ACMII. In step 1, ACM(II)-GCN implement different feature extractions for $3$ channels using a set of filterbanks. Three filtered components, $H_L^l,H_H^l, H_I^l$, are obtained. To adaptively exploit information from each channel, ACM(II)-GCN first extract nonlinear information from the filtered signals, then use $W_\text{Mix}^l$ to learn which channel is important for each node, leading to the row-wise weight vectors $\alpha_L^l,\alpha_H^l,\alpha_I^l \in \mathbb{R}^{N\times 1}$ whose $i$-th elements are the weights for node $i$. These three vectors are then used as weights in defining the updated $H^l$ in step 3.

\subsection{Implementation of ACM-GCNII}
Unlike other baseline GNN models, GCNII and GCNII* are not able to be applied under ACMII framework and we will make an explanation as follows.
\begin{align*}
       & \text{GCNII: } \mathbf{H}^{(\ell+1)}=\sigma\left(\left(\left(1-\alpha_{\ell}\right) \hat{\mathbf{A}} \mathbf{H}^{(\ell)}+\alpha_{\ell} \mathbf{H}^{(0)}\right)\left(\left(1-\beta_{\ell}\right) \mathbf{I}_{n}+\beta_{\ell} \mathbf{W}^{(\ell)}\right)\right)\\
       & \resizebox{1\hsize}{!}{$\text{GCNII*: }
       \mathbf{H}^{(\ell+1)}= \sigma\left(\left(1-\alpha_{\ell}\right) \hat{\mathbf{A}} \mathbf{H}^{(\ell)}\left(\left(1-\beta_{\ell}\right) \mathbf{I}_{n}+\beta_{\ell} \mathbf{W}_{1}^{(\ell)}\right)+\right. \left.+\alpha_{\ell} \mathbf{H}^{(0)}\left(\left(1-\beta_{\ell}\right) \mathbf{I}_{n}+\beta_{\ell} \mathbf{W}_{2}^{(\ell)}\right)\right)$}
\end{align*}
From the above formulas of GCNII and GCNII$^*$ we cam see that, without major modification, GCNII and GCNII* are hard to be put into ACMII framework. In ACMII framework, before apply $\hat{A}$, we first implement a nonlinear feature extractor $\sigma(H^{\ell} \mathbf{W}^{(\ell)})$. But in GCNII and GCNII*, before multiplying $W^\ell (\text{or }W_1^\ell, W_2^\ell)$ to extract features, we need to add another term including $H^{(0)}$, which are not filtered by $\hat{A}$. This makes the order of aggregator $\hat{A}$ and nonlinear extractor unexchangable and thus, incompatible with ACMII framework. So we did not implement GCNII and GCNII* in ACMII framework. 

\subsection{Implementation of ACM(II)-GCN+ and ACM(II)-GCN++}
Besides the features extracted by different filters, some recent SOTA models use additional graph structure information explicitly, i.e., $\text{MLP}_\theta(A)$ , to address heterophily problem, e.g., LINKX \cite{lim2021large} and GloGNN \cite{li2022finding} and is found effective on some datasets, e.g., $\textit{Chameleon, Squirrel}$. The explicit structure information can be directly incorporated into ACM and ACMII framework, and we have ACM(II)-GCN+ and ACM(II)-GCN++.

\textbf{ACM-GCN+ and ACMII-GCN+} have an option to include structure information channel (the 4-th channel) in each layer and their differences from ACM-GCN and ACMII-GCN as follows,
\begin{equation*}
\begin{aligned}
\label{eq:acm_gnn+_spectral}
& \textbf{{Step 1. Feature Extraction for LP, HP, Identity and Structure Information Channel:}} \\
&\resizebox{1\hsize}{!}{${{H}^l_A = \text{ReLU}\left(A W^l_A\right), W^l_A \in \mathbb{R}^{N\times F_l}}, \text{ get ${H}^{l}_L,{H}^{l}_H,{H}^{l}_I$ with the same step as ACM-GCN and ACMII-GCN.} $}\\
& \textbf{Step 2. Row-wise Feature-based Weight Learning with Layer Normalization (LN)} \\
& {\tilde{H}^{l}_L = \text{LN} ({H}^{l}_L),\ \tilde{H}^{l}_H = \text{LN}({H}^{l}_H),\ \tilde{H}^{l}_I = \text{LN}({H}^{l}_I),\ \tilde{H}^l_A = \text{LN}({H}^l_A),} \\
&\resizebox{1\hsize}{!}{$\tilde{\alpha}_L^l = \text{Sigmoid} \left(\tilde{H}^{l}_L \tilde{W}^{l}_L\right),\ \tilde{\alpha}_H^l = \text{Sigmoid} \left(\tilde{H}^{l}_H \tilde{W}^{l}_H\right), \tilde{\alpha}_I^l = \text{Sigmoid} \left(\tilde{H}^{l}_I \tilde{W}^{l}_I\right), \tilde{\alpha}_A^l = \text{Sigmoid} \left(\tilde{H}^l_A \tilde{W}^{l}_A\right), $}
\\
&\tilde{W}_L^{l-1},\ \tilde{W}_H^{l-1},\ \tilde{W}_I^{l-1},\tilde{W}^{l}_A \in \mathbb{R}^{F_l \times 1}\\ 
&\textbf{Step 3. Node-wise Adaptive Channel Mixing:}&\\
& \text{Option 1: without structure information} \\
&\left[{\alpha}_L^l, {\alpha}_H^l, {\alpha}_I^l \right] = \text{Softmax}\left((\left[\tilde{\alpha}_L^l,\tilde{\alpha}_H^l,\tilde{\alpha}_I^l\right]/T) W_\text{Mix}^l \right) \in \mathbb{R}^{N\times 3}, T = 3   \text{ temperature},\ W_\text{Mix}^l \in \mathbb{R}^{3\times 3}; \\
&{H^{l}}  = \text{ReLU}\left( \text{diag}(\alpha_L^l){H}^{l}_L + \text{diag}(\alpha_H^l){H}^{l}_H + \text{diag}(\alpha_I^l){H}^{l}_I\right)\\
& \text{Option 2: with structure information}\\
&\resizebox{1\hsize}{!}{${\left[{\alpha}_L^l, {\alpha}_H^l, {\alpha}_I^l, {\alpha}_A^l \right] = \text{Softmax}\left((\left[\tilde{\alpha}_L^l,\tilde{\alpha}_H^l,\tilde{\alpha}_I^l,\tilde{\alpha}_A^l\right]/T) W_\text{Mix}^l \right) \in \mathbb{R}^{N\times 4}, T = 4 \text{ temperature},\ W_\text{Mix}^l \in \mathbb{R}^{4\times 4};} $} \\
& {{H^{l}}  =  \text{ReLU}\left(\text{diag}(\alpha_L^l){H}^{l}_L + \text{diag}(\alpha_H^l){H}^{l}_H + \text{diag}(\alpha_I^l){H}^{l}_I + \text{diag}(\alpha_A^l){H}^{l}_A \right) }\\
\end{aligned}
\end{equation*}





\section{ACM-GNN Empirical Evaluation}
We evaluate SGC \cite{wu2019simplifying} with 1 hop and 2 hops (SGC-1, SGC-2), GCNII \cite{chen2020simple}, GCNII$^*$ \cite{chen2020simple}, GCN \cite{kipf2016classification} and snowball networks \cite{luan2019break} with 2 and 3 layers (snowball-2, snowball-3) and combine them with the ACM or ACMII framework. We use $\hat{A}_\text{rw}$ as the LP filter and the corresponding HP filter is $I-\hat{A}_\text{rw}$. Both filters are deterministic. We compare these approaches with several baselines and SOTA GNN models: MLP with 2 layers (MLP-2), GAT \cite{velivckovic2017attention},  APPNP \cite{klicpera2018predict}, GPRGNN \cite{chien2021adaptive}, H$_2$GCN \cite{zhu2020beyond}, MixHop \cite{abu2019mixhop}, GCN+JK \cite{kipf2016classification, lim2021new}, GAT+JK \cite{velivckovic2017attention, lim2021new}, FAGCN \cite{bo2021beyond}, GraphSAGE \cite{hamilton2017inductive}, Geom-GCN \cite{pei2020geom} and BernNet \cite{he2021bernnet}. In addition to the 9 benchmark datasets listed in Sec.~\ref{sec:acm.ablation.study}, we further test the above models on a new benchmark dataset, \textit{Deezer-Europe} \cite{feather}.

On each dataset used in \cite{pei2020geom}, we test the models 10 times following the same early stopping strategy, the same 60\%/20\%/20\% random data split and optimizer as used in GPRGNN \cite{chien2021adaptive}. In addition, we show the performance comparison with several SOTA models, e.g., LINKX \cite{lim2021large} and GloGNN \cite{li2022finding}, on the fixed 48\%/32\%/20\% splits provided by \cite{pei2020geom}.

Besides the filtered features, some recent SOTA models additionally use graph structure information, i.e., $\text{MLP}_\theta(A)$, and residual connection to address heterophily problem, e.g., LINKX \cite{lim2021large} and GloGNN \cite{li2022finding}. $\text{MLP}_\theta(A)$ and residual connection can be directly incorporated into ACM and ACMII framework, which leads us to ACM(II)-GCN+ and ACM(II)-GCN++.

\begin{figure}[ht!]
    \centering
     {
    \subfloat[ Input Feature]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/squirrel_features.pdf}
     } 
     \subfloat[GCN Output]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/squirrel_gcn.pdf}
     } 
     \subfloat[ACM-GCN Output]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/squirrel_3channel_all.pdf}
     } \\
     
     \subfloat[Low-pass Channel]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.22\textwidth]{Images1/squirrel_3channel_low.pdf}
     } 
     \subfloat[High-pass Channel]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.22\textwidth]{Images1/squirrel_3channel_high.pdf}
     } 
     \subfloat[Identity Channel]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.22\textwidth]{Images1/squirrel_3channel_mlp.pdf}
     }
     \subfloat[Learned Weights ${\alpha}$]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.22\textwidth]{Images1/alpha_squirrel.pdf}
     } 
     }
     \caption{t-SNE visualization of the output of ACM-GCN and GCN trained on Squirrel}
     \label{fig:visualization_acmgcn}
\end{figure}
\subsection{Ablation Study}
\label{sec:acm.ablation.study}
We investigate the effectiveness and efficiency of adding HP, identity channels and the adaptive mixing mechanism in the proposed framework by performing an ablation study.
Specifically, we apply the components of ACM to SGC-1 \cite{wu2019simplifying} \footnote{We only test ACM-SGC-1 because SGC-1 does not contain any non-linearity which makes ACM-SGC-1 and ACMII-SGC-1 exactly the same.} and the components of ACM and ACMII to GCN \cite{kipf2016classification} separately. 
We run 10 times on each of the 9 benchmark datatsets, \textit{Cornell}, \textit{Wisconsin}, \textit{Texas}, \textit{Film}, \textit{Chameleon}, \textit{Squirrel}, \textit{Cora}, \textit{Citeseer} and \textit{Pubmed} used in \cite{pei2020geom}, with the same 60\%/20\%/20\% random splits for train/validation/test used in \cite{chien2021adaptive} and report the average test accuracy as well as the standard deviation. 
We also record the average running time per epoch (in milliseconds) to compare the computational efficiency. 
We set the temperature $T$ in Eq.~\ref{eq:acm_gnn_spectral} to be $3$, which is the number of channels.
\input{Tables1/acm.ablation.study.tex}

The results in Tab.~\ref{tab:ablation.study} show that on most datasets, the additional HP and identity channels are helpful, even for strong homophily datasets such as \textit{Cora, CiteSeer and PubMed}. The adaptive mixing mechanism also has an advantage over directly adding the three channels together. This illustrates the necessity of learning to customize the channel usage adaptively for different nodes. The t-SNE visualization in Fig.~\ref{fig:visualization_acmgcn} demonstrates that the high-pass channel(e) and identity channel(f) can extract meaningful patterns, which the low-pass channel(d) is not able to capture. The output of ACM-GCN(c) shows clearer boundaries among classes than GCN(b). The running time is approximately doubled in the ACM and ACMII framework compared to the original models.

\input{Tables1/acm.sota.comparison.random.split.tex}
\subsection{Comparison with SOTA on 60\%/20\%/20\% Random Splits}
\label{sec:acm.sota.fix.split}
The main results of the full sets of experiments with statistics of datasets are summarized in Tab.~\ref{tab:acm.sota.random.split}, where we report the mean accuracy (\%) and standard deviation. We can see that after applied in ACM or ACMII framework, the performance of baseline models are boosted on almost all tasks and achieve SOTA performance on $9$ out of $10$ datasets. Especially, ACMII-GCN+ performs the best in terms of average rank (4.40) across all datasets. Overall, It suggests that ACM or ACMII framework can significantly increase the performance of GNNs on node classification tasks on heterophilic graphs and maintain highly competitive performance on homophilic datasets.

\subsection{Comparison with SOTA on 48\%/32\%/20\% Fixed Splits}
\input{Tables1/acm.sota.comparison.fixed.split}
The main results of the full sets of experiments with statistics of datasets are summarized in Tab.~\ref{tab:acm.sota.fixed.split}, where we report the mean accuracy (\%) and standard deviation. We can see that after applied in ACM or ACMII framework, the performance of baseline models are boosted on almost all tasks and achieve SOTA performance on $4$ out of $10$ datasets. Especially, ACMII-GCN++ performs the best in terms of average rank (4.78) across all datasets. Overall, It suggests that ACM or ACMII framework can significantly increase the performance of GNNs on node classification tasks on heterophilic graphs and maintain highly competitive performance on homophilic datasets.

\subsection{Comparison with SOTA on Large-Scale Datasets}
\input{Tables1/acm.sota.comparison.large}
The main results of the full sets of experiments with statistics of datasets are summarized in Tab.~\ref{tab:acm.sota.large.scale}, where we report the mean accuracy (\%) and standard deviation. We can see that after applied in ACM or ACMII framework, the performance of baseline models are boosted on almost all tasks and achieve SOTA performance on $2$ out of $4$ datasets. Especially, ACM-GCN++ performs the best in terms of average rank (2.5) across all datasets. Overall, It suggests that ACM or ACMII framework can significantly increase the performance of GNNs on node classification tasks on heterophilic graphs and maintain highly competitive performance on homophilic datasets.

\begin{figure}[htbp!]
    \centering
     {
    \subfloat[ \texttt{Cornell}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_cornell.pdf}
     } 
     \subfloat[ \texttt{Wisconsin}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_wisconsin.pdf}
     } 
     \subfloat[ \texttt{Texas}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_texas.pdf}
     } \\
     \subfloat[ \texttt{Chameleon}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_chameleon.pdf}
     } 
     \subfloat[ \texttt{Squirrel}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_squirrel.pdf}
     } 
     \subfloat[ \texttt{Film}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_film.pdf}
     } \\
     \subfloat[ \texttt{Cora}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_cora.pdf}
     } 
     \subfloat[ \texttt{Citeseer}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_citeseer.pdf}
     } 
     \subfloat[ \texttt{Pubmed}]{
     \captionsetup{justification = centering}
     \includegraphics[width=0.3\textwidth]{Images1/alpha_pubmed.pdf}
     } 
     }
     \caption{Distributions of the learned $\alpha_L, \alpha_H, \alpha_I$  in the output layer of ACM-GCN}
     \label{fig:Alpha_values_output_layer}
\end{figure}
\subsection{Distributions of Mixing Weights of ACM-GCN}
In Fig.~\ref{fig:Alpha_values_output_layer}, we illustrate the distributions of mixing weights $\alpha_L, \alpha_H, \alpha_I$ in output layers of ACM-GCN. With the node local homophily distributions in Fig.~\ref{fig:local_homo_distributions} as the reference, we can see that our adaptive channel mixing GNN framework can successfully learn from homophilic and heterophilic signals for graphs at different homophily levels.

\section{Conclusions and Limitations}
We have presented an analysis of existing homophily metrics and proposed new metrics which are more informative in terms of correlating with GNN performance. 
 To our knowledge, this is the first work analyzing heterophily from the perspective of post-aggregation node similarity.
 The similarity matrix and the new metrics we defined  mainly capture linear feature-independent relationships of each node. This might be insufficient when nonlinearity and feature-dependent information is important for classification. In the future, it would be useful to investigate if a similarity matrix could be defined which is capable of capturing nonlinear and feature-dependent relations between aggregated node.

%The metrics defined in \eqref{eq:aggregation_similarity} are found to be insensitive in high-homophily area and over-sensitive in low-homophily area. This will impair the practical value of the proposed metrics. New homophily metrics should be investigated to provide better guidance on how graph structure will influence the performance of GNNs.

We have also proposed a multi-channel mixing mechanism which leverages the intuitions gained in the first part of the paper and can be combined with different GNN architectures, enabling adaptive filtering (high-pass, low-pass or identity) at different nodes. Empirically, this approach shows very promising results, improving the performance of the base GNNs with which it is combined and achieving SOTA results at the cost of a reasonable increase in computation time.
As discussed in Sec.~\ref{sec:filterbank_acm_gnn_architecture}, however, the filterbank method cannot properly handle all cases of harmful  heterophily, and alternative ideas should be explored as well in the future.

This chapter concludes for the designs of GNNs for node-level classification on homophilic and heterophilic graph datasets. In the next chapter, we introduce GNNs with high-order pooling functions for graph-level classification.


==> Tables1/acm.ablation.study.tex <==
\begin{table*}[htbp]
  \centering
  \setlength{\tabcolsep}{1pt}
   \resizebox{1\hsize}{!}{
    \begin{tabular}{c|cccc|ccccccccc|r}
    \toprule
    \toprule
    \multicolumn{14}{c}{Ablation Study on Different Components in ACM-SGC and ACM-GCN (\%)}                       &  \\
    \midrule
    \multicolumn{1}{p{4.125em}|}{Baseline    } & \multicolumn{4}{c|}{Model Components} & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Cora  & CiteSeer & PubMed & \multicolumn{1}{c}{\multirow{1}[4]{*}{Rank}} \\
\cmidrule{2-14}    \multicolumn{1}{p{4.125em}|}{Models} & LP    & HP    & Identity & Mixing & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std & Acc $\pm$ Std &  \\
    \midrule
    \multicolumn{1}{c|}{\multirow{5}[1]{*}{ACM-SGC-1 w/}} & $\checkmark$ &       &       &       & 70.98 $\pm$ 8.39 & 70.38 $\pm$ 2.85 & 83.28 $\pm$ 5.43 & 25.26 $\pm$ 1.18 & 64.86 $\pm$ 1.81 & 47.62 $\pm$ 1.27 & 85.12 $\pm$ 1.64 & 79.66 $\pm$ 0.75 & 85.5 $\pm$ 0.76 & \multicolumn{1}{c}{12.89} \\
          & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 83.28 $\pm$ 5.81 & 91.88 $\pm$ 1.61 & 90.98 $\pm$ 2.46 & 36.76 $\pm$ 1.01 & 65.27 $\pm$ 1.9 & 47.27 $\pm$ 1.37 & 86.8 $\pm$ 1.08 & 80.98 $\pm$ 1.68 & 87.21 $\pm$ 0.42 & \multicolumn{1}{c}{10.44} \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 93.93 $\pm$ 3.6 & 95.25 $\pm$ 1.84 & 93.93 $\pm$ 2.54 & 38.38 $\pm$ 1.13 & 63.83 $\pm$ 2.07 & 46.79 $\pm$ 0.75 & 86.73 $\pm$ 1.28 & 80.57 $\pm$ 0.99 & 87.8 $\pm$ 0.58 & \multicolumn{1}{c}{9.44} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 88.2 $\pm$ 4.39 & 93.5 $\pm$ 2.95 & 92.95 $\pm$ 2.94 & 37.19 $\pm$ 0.87 & 62.82 $\pm$ 1.84 & 44.94 $\pm$ 0.93 & 85.22 $\pm$ 1.35 & 80.75 $\pm$ 1.68 & 88.11 $\pm$ 0.21 & \multicolumn{1}{c}{11.00} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 93.77 $\pm$ 1.91 & 93.25 $\pm$ 2.92 & 93.61 $\pm$ 1.55 & 39.33 $\pm$ 1.25 & 63.68 $\pm$ 1.62 & 46.4 $\pm$ 1.13 & 86.63 $\pm$ 1.13 & 80.96 $\pm$ 0.93 & 87.75 $\pm$ 0.88 & \multicolumn{1}{c}{10.00} \\
          \midrule
    \multicolumn{1}{c|}{\multirow{5}[0]{*}{ACM-GCN w/}} & $\checkmark$ &       &       &       & 82.46 $\pm$ 3.11 & 75.5 $\pm$ 2.92 & 83.11 $\pm$ 3.2 & 35.51 $\pm$ 0.99 & 64.18 $\pm$ 2.62 & 44.76 $\pm$ 1.39 & 87.78 $\pm$ 0.96 & 81.39 $\pm$ 1.23 & 88.9 $\pm$ 0.32 & \multicolumn{1}{c}{11.44} \\
          & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 82.13 $\pm$ 2.59 & 86.62 $\pm$ 4.61 & 89.19 $\pm$ 3.04 & 38.06 $\pm$ 1.35 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{69.21 $\pm$ 1.68} & 57.2 $\pm$ 1.01 & 88.93 $\pm$ 1.55 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{81.96 $\pm$ 0.91} & 90.01 $\pm$ 0.8  & \multicolumn{1}{c}{7.22} \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 94.26 $\pm$ 2.23 & 96.13 $\pm$ 2.2 & 94.1 $\pm$ 2.95 & 41.51 $\pm$ 0.99 & 67.44 $\pm$ 2.14 & 53.97 $\pm$ 1.39 & 88.95 $\pm$ 0.9 & 81.72 $\pm$ 1.22 & 90.88 $\pm$ 0.55 & \multicolumn{1}{c}{4.44} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 91.64 $\pm$ 2 & 95.37 $\pm$ 3.31 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{95.25 $\pm$ 2.37} & 40.47 $\pm$ 1.49 & 68.93 $\pm$ 2.04 & 54.78 $\pm$ 1.27 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{89.13 $\pm$ 1.77} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{81.96 $\pm$ 2.03} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{91.01 $\pm$ 0.7} & \multicolumn{1}{c}{3.11} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 94.75 $\pm$ 2.62 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{96.75 $\pm$ 1.6} & 95.08 $\pm$ 3.2 & 41.62 $\pm$ 1.15 & 69.04 $\pm$ 1.74 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{58.02 $\pm$ 1.86} & 88.95 $\pm$ 1.3 & 81.80 $\pm$ 1.26 & 90.69 $\pm$ 0.53 & \multicolumn{1}{c}{\cellcolor[rgb]{ .816,  .808,  .808}\textbf{2.78}} \\
          \midrule
    \multicolumn{1}{c|}{\multirow{4}[1]{*}{ACMII-GCN w/}} & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 82.46 $\pm$ 3.03 & 91.00 $\pm$ 1.75 & 90.33 $\pm$ 2.69 & 38.39 $\pm$ 0.75 & 67.59 $\pm$ 2.14 & 53.67 $\pm$ 1.71 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{89.13 $\pm$ 1.14} & 81.75 $\pm$ 0.85 & 89.87 $\pm$ 0.39 & \multicolumn{1}{c}{7.44} \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 94.26 $\pm$ 2.57 & 96.00 $\pm$ 2.15 & 94.26 $\pm$ 2.96 & 40.96 $\pm$ 1.2 & 66.35 $\pm$ 1.76 & 50.78 $\pm$ 2.07 & 89.06 $\pm$ 1.07 & 81.86 $\pm$ 1.22 & 90.71 $\pm$ 0.67 & \multicolumn{1}{c}{4.67} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 91.48 $\pm$ 1.43 & 96.25 $\pm$ 2.09 & 93.77 $\pm$ 2.91 & 40.27 $\pm$ 1.07 & 66.52 $\pm$ 2.65 & 52.9 $\pm$ 1.64 & 88.83 $\pm$ 1.16 & 81.54 $\pm$ 0.95 & 90.6 $\pm$ 0.47 & \multicolumn{1}{c}{6.67} \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{95.9 $\pm$ 1.83} & 96.62 $\pm$ 2.44 & 95.25 $\pm$ 3.15 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{41.84 $\pm$ 1.15} & 68.38 $\pm$ 1.36 & 54.53 $\pm$ 2.09 & 89.00 $\pm$ 0.72 & 81.79 $\pm$ 0.95 & 90.74 $\pm$ 0.5 & \multicolumn{1}{c}{\cellcolor[rgb]{ .816,  .808,  .808}\textbf{2.78}} \\
\cmidrule{1-14}    \multicolumn{14}{c|}{Comparison of Average Running Time Per Epoch(ms)}                                        &  \\
\cmidrule{1-14}    \multicolumn{1}{c|}{\multirow{5}[2]{*}{ACM-SGC-1 w/}} & $\checkmark$ &       &       &       & 2.53  & 2.83  & 2.5   & 3.18  & 3.48  & 4.65  & 3.47  & 3.43  & 4.04  &  \\
          & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 4.01  & 4.57  & 4.24  & 4.55  & 4.76  & 5.09  & 5.39  & 4.69  & 4.75  &  \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 3.88  & 4.01  & 4.04  & 4.43  & 4.06  & 4.5   & 4.38  & 3.82  & 4.16  &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 3.31  & 3.49  & 3.18  & 3.7   & 3.53  & 4.83  & 3.92  & 3.87  & 4.24  &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 5.53  & 5.96  & 5.43  & 5.21  & 5.41  & 6.96  & 6     & 5.9   & 6.04  &  \\
\cmidrule{1-14}    \multicolumn{1}{c|}{\multirow{5}[2]{*}{ACM-GCN w/}} & $\checkmark$ &       &       &       & 3.67  & 3.74  & 3.59  & 4.86  & 4.96  & 6.41  & 4.24  & 4.18  & 5.08  &  \\
          & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 6.63  & 8.06  & 7.89  & 8.11  & 7.8   & 9.39  & 7.82  & 7.38  & 8.74  &  \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 5.73  & 5.91  & 5.93  & 6.86  & 6.35  & 7.15  & 7.34  & 6.65  & 6.8   &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 5.16  & 5.25  & 5.2   & 5.93  & 5.64  & 8.02  & 5.73  & 5.65  & 6.16  &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 8.25  & 8.11  & 7.89  & 7.97  & 8.41  & 11.9  & 8.84  & 8.38  & 8.63  &  \\
\cmidrule{1-14}    \multicolumn{1}{c|}{\multirow{4}[2]{*}{ACMII-GCN w/}} & $\checkmark$ & $\checkmark$ &       & $\checkmark$ & 6.62  & 7.35  & 7.39  & 7.62  & 7.33  & 9.69  & 7.49  & 7.58  & 7.97  &  \\
          & $\checkmark$ &       & $\checkmark$ & $\checkmark$ & 6.3   & 6.05  & 6.26  & 6.87  & 6.44  & 6.5   & 6.14  & 7.21  & 6.6   &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ &       & 5.24  & 5.27  & 5.46  & 5.72  & 5.65  & 7.87  & 5.48  & 5.65  & 6.33  &  \\
          & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 7.59  & 8.28  & 8.06  & 8.85  & 8     & 10    & 8.27  & 8.5   & 8.68  &  \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
    \caption{Ablation study on 9 real-world datasets \cite{pei2020geom}. Cell with \checkmark means the component is applied to the baseline model. The best test results are highlighted.}
     \label{tab:ablation.study}
\end{table*}%

==> Tables1/acm.sota.comparison.fixed.split.tex <==
% Table generated by Excel2LaTeX from sheet 'Fixed Splits'
\begin{table}[htbp]
  \centering
  \setlength{\tabcolsep}{3pt}
    \resizebox{1\hsize}{!}{
    \begin{tabular}{c|ccccccccc|c}
    \toprule
    \toprule
    Datasets/Models & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Cora  & Citeseer & PubMed & Average Rank \\
    \midrule
    Geom-GCN & 60.54 $\pm$ 3.67 & 64.51 $\pm$ 3.66 & 66.76 $\pm$ 2.72 & 31.59 $\pm$ 1.15 & 60.00 $\pm$ 2.81 & 38.15 $\pm$ 0.92 & 85.35 $\pm$ 1.57 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{78.02 $\pm$ 1.15} & 89.95 $\pm$ 0.47 & 18.22 \\
    H2GCN & 82.70 $\pm$ 5.28 & 87.65 $\pm$ 4.98 & 84.86 $\pm$ 7.23 & 35.70 $\pm$ 1.00 & 60.11 $\pm$ 2.15 & 36.48 $\pm$ 1.86 & 87.87 $\pm$ 1.20 & 77.11 $\pm$ 1.57 & 89.49 $\pm$ 0.38 & 15.11 \\
    GPRGCN & 78.11 $\pm$ 6.55 & 82.55 $\pm$ 6.23 & 81.35 $\pm$ 5.32 & 35.16 $\pm$ 0.9 & 62.59 $\pm$ 2.04 & 46.31 $\pm$ 2.46 & 87.95 $\pm$ 1.18 & 77.13 $\pm$ 1.67 & 87.54 $\pm$ 0.38 & 17.67 \\
    FAGCN & 76.76 $\pm$ 5.87 & 79.61 $\pm$ 1.58 & 76.49 $\pm$ 2.87 & 34.82 $\pm$ 1.35 & 46.07 $\pm$ 2.11 & 30.83 $\pm$ 0.69 & 88.05 $\pm$ 1.57 & 77.07 $\pm$ 2.05 & 88.09 $\pm$ 1.38 & 20.00 \\
    GCNII & 77.86 $\pm$ 3.79  & 80.39 $\pm$ 3.40 & 77.57 $\pm$ 3.83 & 37.44 $\pm$ 1.30 & 63.86 $\pm$ 3.04  & 38.47 $\pm$ 1.58 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.37 $\pm$ 1.25 } & 77.33 $\pm$ 1.48 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{90.15 $\pm$ 0.43} & 12.44 \\
    MixHop & 73.51 $\pm$ 6.34  & 75.88 $\pm$ 4.90  & 77.84 $\pm$ 7.73  & 32.22 $\pm$ 2.34 & 60.50 $\pm$ 2.53  &  43.80 $\pm$ 1.48  & 87.61 $\pm$ 0.85  & 76.26 $\pm$1.33  & 85.31 $\pm$ 0.61 & 20.78 \\
    WRGAT & 81.62 $\pm$3.90  & 86.98 $\pm$ 3.78  & 83.62 $\pm$ 5.50  & 36.53 $\pm$ 0.77  & 65.24 $\pm$ 0.87  & 48.85 $\pm$ 0.78 & 88.20 $\pm$ 2.26  & 76.81 $\pm$ 1.89  & 88.52 $\pm$ 0.92 & 14.33 \\
    GGCN  & 85.68 $\pm$ 6.63  & 86.86 $\pm$ 3.29  & 84.86 $\pm$ 4.55 & 37.54 $\pm$ 1.56  & 71.14 $\pm$1.84  & 55.17 $\pm$ 1.58 & 87.95 $\pm$ 1.05  & 77.14 $\pm$ 1.45  & 89.15 $\pm$ 0.37 & 10.22 \\
    LINKX &  77.84 $\pm$ 5.81  & 75.49 $\pm$ 5.72 & 74.60 $\pm$ 8.37  & 36.10 $\pm$ 1.55  & 68.42 $\pm$ 1.38  & 61.81 $\pm$ 1.80 & 84.64 $\pm$ 1.13 & 73.19 $\pm$ 0.99 & 87.86 $\pm$ 0.77 & 18.78 \\
    GloGNN & 83.51 $\pm$ 4.26 & 87.06 $\pm$ 3.53  & 84.32 $\pm$ 4.15  & 37.35 $\pm$ 1.30 & 69.78 $\pm$ 2.42  & 57.54 $\pm$ 1.39  & 88.31 $\pm$ 1.13 & 77.41 $\pm$ 1.65  & 89.62 $\pm$ 0.35 & 8.78 \\
    GloGNN++ & 85.95 $\pm$ 5.10  &  88.04 $\pm$ 3.22  & 84.05 $\pm$ 4.90 & 37.70 $\pm$ 1.40  & 71.21 $\pm$ 1.84  & 57.88 $\pm$ 1.76  & 88.33 $\pm$ 1.09  & 77.22 $\pm$ 1.78  & 89.24 $\pm$ 0.39 & 7.33 \\
    ACM-SGC-1 & 82.43 $\pm$ 5.44 & 86.47 $\pm$ 3.77 & 81.89 $\pm$ 4.53 & 35.49 $\pm$ 1.06 & 63.99 $\pm$ 1.66 & 45.00 $\pm$ 1.4 & 86.9 $\pm$ 1.38 & 76.73 $\pm$ 1.59 & 88.49 $\pm$ 0.51 & 17.56 \\
    ACM-SGC-2 & 82.43 $\pm$ 5.44 & 86.47 $\pm$ 3.77 & 81.89 $\pm$ 4.53 & 36.04 $\pm$ 0.83 & 59.21 $\pm$ 2.22 & 40.02 $\pm$ 0.96 & 87.69 $\pm$ 1.07 & 76.59 $\pm$ 1.69 & 89.01 $\pm$ 0.6 & 17.67 \\
    Diag-NSD & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{86.49 $\pm$ 7.35} & 88.63 $\pm$ 2.75 & 85.67 $\pm$ 6.95 & 37.79 $\pm$ 1.01 & 68.68 $\pm$ 1.73 & 54.78 $\pm$ 1.81 & 87.14 $\pm$ 1.06 & 77.14 $\pm$ 1.85 & 89.42 $\pm$ 0.43 & 9.00 \\
    O(d)-NSD & 84.86 $\pm$ 4.71 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{89.41 $\pm$ 4.74} & 85.95 $\pm$ 5.51 & 37.81 $\pm$ 1.15 & 68.04 $\pm$ 1.58 & 56.34 $\pm$ 1.32 & 86.90 $\pm$ 1.13 & 76.70 $\pm$ 1.57 & 89.49 $\pm$ 0.40 & 10.44 \\
    Gen-NSD & 85.68 $\pm$ 6.51 & 89.21 $\pm$ 3.84 & 82.97 $\pm$ 5.13  & 37.80 $\pm$ 1.22 & 67.93 $\pm$ 1.58 & 53.17 $\pm$ 1.31 & 87.30 $\pm$ 1.15 & 76.32 $\pm$ 1.65 & 89.33 $\pm$ 0.35 & 11.67 \\
    NLMLP  & 84.9 $\pm$ 5.7 & 87.3 $\pm$ 4.3  & 85.4 $\pm$ 3.8 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{37.9 $\pm$ 1.3} & 50.7 $\pm$ 2.2 & 33.7 $\pm$ 1.5 & 76.9 $\pm$ 1.8 & 73.4 $\pm$ 1.9 & 88.2 $\pm$ 0.5 & 16.67 \\
    NLGCN  & 57.6 $\pm$ 5.5 & 60.2 $\pm$ 5.3  & 65.5 $\pm$ 6.6 & 31.6 $\pm$ 1.0 & 70.1 $\pm$ 2.9 & 59.0 $\pm$ 1.2 & 88.1 $\pm$ 1.0 & 75.2 $\pm$ 1.4 & 89.0 $\pm$ 0.5 & 17.44 \\
    NLGAT  & 54.7 $\pm$ 7.6 & 56.9 $\pm$ 7.3 & 62.6 $\pm$ 7.1 & 29.5 $\pm$ 1.3 & 65.7 $\pm$ 1.4 & 56.8 $\pm$ 2.5 & 88.5 $\pm$ 1.8 & 76.2 $\pm$ 1.6 & 88.2 $\pm$ 0.3 & 18.56 \\
    \midrule
    ACM-GCN & 85.14 $\pm$ 6.07 & 88.43 $\pm$ 3.22 & 87.84 $\pm$ 4.4 & 36.63 $\pm$ 0.84 & 69.14 $\pm$ 1.91 & 55.19 $\pm$ 1.49 & 87.91 $\pm$ 0.95 & 77.32 $\pm$ 1.7 & 90.00 $\pm$ 0.52 & 8.11 \\
    ACMII-GCN & 85.95 $\pm$ 5.64 & 87.45 $\pm$ 3.74 & 86.76 $\pm$ 4.75 & 36.31 $\pm$ 1.2 & 68.46 $\pm$ 1.7 & 51.8 $\pm$ 1.5 & 88.01 $\pm$ 1.08 & 77.15 $\pm$ 1.45 & 89.89 $\pm$ 0.43 & 9.33 \\
    ACM-GCN+ & 85.68 $\pm$ 4.84 & 88.43 $\pm$ 2.39 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.38 $\pm$ 3.64} & 36.26 $\pm$ 1.34 & 74.47 $\pm$ 1.84 & 66.98 $\pm$ 1.71 & 88.05 $\pm$ 0.99 & 77.67 $\pm$ 1.19 & 89.82 $\pm$ 0.41 & 5.33 \\
    ACMII-GCN+ & 85.41 $\pm$ 5.3 & 88.04 $\pm$ 3.66 & 88.11 $\pm$ 3.24 & 36.14 $\pm$ 1.44 & 74.56 $\pm$ 2.08 & 67.07 $\pm$ 1.65 & 88.19 $\pm$ 1.17 & 77.2 $\pm$ 1.61 & 89.78 $\pm$ 0.49  & 6.78 \\
    ACM-GCN++ & 85.68 $\pm$ 5.8 & 88.24 $\pm$ 3.16 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.38 $\pm$ 3.43} & 37.31 $\pm$ 1.09 & 74.41 $\pm$ 1.49 & 67.06 $\pm$ 1.66 & 88.11 $\pm$ 0.96 & 77.46 $\pm$ 1.65 & 89.65 $\pm$ 0.58 & 5.33 \\
    ACMII-GCN++ & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{86.49 $\pm$ 6.73} & 88.43 $\pm$ 3.66 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.38 $\pm$ 3.43} & 37.09 $\pm$ 1.32 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{74.76 $\pm$ 2.2} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{67.4 $\pm$ 2.21} & 88.25 $\pm$ 0.96 & 77.12 $\pm$ 1.58 & 89.71 $\pm$ 0.48 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{4.78} \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
    \caption{Experimental results on fixed splits provided by \cite{pei2020geom}: average test accuracy $\pm$ standard deviation on 9 real-world benchmark datasets. The best results are highlighted. Results of Geom-GCN, H$_2$GCN and GPRGNN, LINX, GloGNN, GloGNN++, Diag-NSD, O(d)-NSD, Gen-NSD, NLMLP, NLGCN and NLGAT are from \cite{pei2020geom,zhu2020beyond,lingam2021simple, lim2021new,li2022finding, bodnar2022neural, liu2021non}.}
  \label{tab:acm.sota.fixed.split}%
\end{table}%


==> Tables1/acm.sota.comparison.large.tex <==
% Table generated by Excel2LaTeX from sheet 'Large Scale'
\begin{table}[ht!]
  \centering
    \resizebox{1\hsize}{!}{
    \begin{tabular}{c|cccc|c}
    \toprule
    \toprule
    Datasets/Models & Penn94 &  arXiv-year &  genius &  twitch-gamers & Average Rank \\
    \midrule
    MLP   & 73.61 $\pm$ 0.40 & 36.70 $\pm$ 0.21 & 86.68 $\pm$ 0.09 & 60.92 $\pm$ 0.07 & 20.75 \\
    L Prop 1-hop &  63.21 $\pm$ 0.39 &  43.42 $\pm$ 0.17 &  66.02 $\pm$ 0.16  & 62.77 $\pm$ 0.24 & 21.75 \\
    L Prop 2-hop &  74.13 $\pm$ 0.46 &  46.07 $\pm$ 0.15 &  67.04 $\pm$ 0.20  & 63.88 $\pm$ 0.24 & 18.00 \\
    LINK  & 80.79 $\pm$ 0.49  &  53.97 $\pm$ 0.18 &  73.56 $\pm$ 0.14 &  64.85 $\pm$ 0.21 & 13.00 \\
    SGC 1-hop &  66.79 $\pm$ 0.27 & 32.83 $\pm$ 0.13 &  82.36 $\pm$ 0.37 &  58.97 $\pm$ 0.19 & 23.25 \\
    SGC 2-hop &  76.09 $\pm$ 0.45 &  32.27 $\pm$ 0.06 &  82.10 $\pm$ 0.14 &  59.94 $\pm$ 0.21 & 21.50 \\
    C\&S 1-hop  & 74.28 $\pm$ 1.19 &  44.51 $\pm$ 0.16 &  82.93 $\pm$ 0.15 &  64.86 $\pm$ 0.27 & 17.50 \\
    C\&S 2-hop &  78.40 $\pm$ 3.12 & 49.78 $\pm$ 0.26 &  84.94 $\pm$ 0.49 &  65.02 $\pm$ 0.16 & 13.75 \\
    GCN   & 82.47 $\pm$ 0.27 &  46.02 $\pm$ 0.26 &  87.42 $\pm$ 0.37 &  62.18 $\pm$ 0.26 & 13.75 \\
    GAT   & 81.53 $\pm$ 0.55 &  46.05 $\pm$ 0.51 &  55.80 $\pm$ 0.87 &  59.89 $\pm$ 4.12 & 18.75 \\
    GCNJK &  81.63 $\pm$ 0.54 &  46.28 $\pm$ 0.29 &  89.30 $\pm$ 0.19 &  63.45 $\pm$ 0.22 & 13.00 \\
    GATJK &  80.69 $\pm$ 0.36  & 45.80 $\pm$ 0.72 & 56.70 $\pm$ 2.07 &  59.98 $\pm$ 2.87 & 19.75 \\
    APPNP &  74.33 $\pm$ 0.38 &  38.15 $\pm$ 0.26 &  85.36 $\pm$ 0.62  & 60.97 $\pm$ 0.10 & 19.75 \\
    GCNII & 82.92 $\pm$ 0.59 &  47.21 $\pm$ 0.28 & 90.24 $\pm$ 0.09  & 63.39 $\pm$ 0.61 & 11.50 \\
    MixHop & 83.47 $\pm$ 0.71 &  51.81 $\pm$ 0.17  & 90.58 $\pm$ 0.16  & 65.64 $\pm$ 0.27 & 8.75 \\
    H2GCN & 81.31 $\pm$ 0.60 &  49.09 $\pm$ 0.10 &  OOM  &  OOM  & 13.50 \\
    GPRGCN & 81.38 $\pm$ 0.16 &  45.07 $\pm$ 0.21 &  90.05 $\pm$ 0.31 &  61.89 $\pm$ 0.29 & 15.50 \\
    WRGAT & 74.32 $\pm$ 0.53 &  OOM  &  OOM  &  OOM  & 21.00 \\
    GGCN  &  OOM  &  OOM  &  OOM  &  OOM  & NA \\
    LINKX & 84.71 $\pm$ 0.52 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{ 56.00 $\pm$ 1.34} &  90.77 $\pm$ 0.27 &  66.06 $\pm$ 0.19 & 5.25 \\
    GloGNN & 85.57 $\pm$ 0.35 &  54.68 $\pm$ 0.34  &  90.66 $\pm$ 0.11 &  66.19 $\pm$ 0.29 & 5.00 \\
    GloGNN++ & 85.74 $\pm$ 0.42 &  54.79 $\pm$ 0.25 &  90.91 $\pm$ 0.13 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{ 66.34 $\pm$ 0.29} & 3.25 \\
    \midrule
    ACM-GCN & 82.73 $\pm$ 0.52 & 44.3 $\pm$ 0.51 & 91.44 $\pm$ 0.08 & 63.92 $\pm$ 0.19  & 10.33 \\
    ACMII-GCN & 82.4 $\pm$ 0.48 & 44.21 $\pm$ 0.19 & 91.19 $\pm$ 0.16 & 63.73 $\pm$ 0.13 & 12.33 \\
    ACM-GCN+ & 85.05 $\pm$  0.19 & 52.45 $\pm$ 0.31 & 91.22 $\pm$0.17  & 66.24 $\pm$ 0.24 & 4.25 \\
    ACMII-GCN+ & 84.95. $\pm$ 0.43 & 52.49 $\pm$ 0.23 & 91.13 $\pm$0.11  & 65.84 $\pm$ 0.15 & 6.00 \\
    ACM-GCN++ & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{86.08 $\pm$ 0.43} & 53.23 $\pm$ 0.55 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{91.37 $\pm$0.23 } & 66.24 $\pm$ 0.28 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{2.5} \\
    ACMII-GCN++ & 85.95 $\pm$ 0.26 & 52.1 $\pm$ 0.26 & 91.01 $\pm$0.22  & 65.92 $\pm$ 0.14 & 5.50 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
    \caption{Comparison on Large-scale Datasets with SOTA.}
  \label{tab:acm.sota.large.scale}%
\end{table}%


==> Tables1/acm.sota.comparison.random.split.tex <==
% Table generated by Excel2LaTeX from sheet 'Results'
\begin{table}[h!]
  \centering
  \setlength{\tabcolsep}{0.5pt}
  \resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccc|c}
    \toprule
    \toprule
          & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Deezer-Europe & Cora  & CiteSeer & PubMed &  \\
    \midrule
    \#nodes & 183   & 251   & 183   & 7,600 & 2,277 & 5,201 & 28,281 & 2,708 & 3,327 & 19,717 &  \\
    \#edges & 295   & 499   & 309   & 33,544 & 36,101 & 217,073 & 92,752 & 5,429 & 4,732 & 44,338 &  \\
    \#features & 1,703 & 1,703 & 1,703 & 931   & 2,325 & 2,089 & 31,241 & 1,433 & 3,703 & 500   &  \\
    \#classes & 5     & 5     & 5     & 5     & 5     & 5     & 2     & 7     & 6     & 3     &  \\
    $H_\text{edge}$ & 0.5669 & 0.4480 & 0.4106 & 0.3750 & 0.2795 & 0.2416 & 0.5251 & 0.8100 & 0.7362 & 0.8024 &  \\
    $H_\text{node}$ & 0.3855 & 0.1498 & 0.0968 & 0.2210 & 0.2470 & 0.2156 & 0.5299 & 0.8252 & 0.7175 & 0.7924 &  \\
    $H_\text{class}$ & 0.0468 & 0.0941 & 0.0013 & 0.0110 & 0.0620 & 0.0254 & 0.0304 & 0.7657 & 0.6270 & 0.6641 &  \\
    Data Splits & 60\%/20\%/20\% & 60\%/20\%/20\% & 60\%/20\%/20\% & 60\%/20\%/20\% & 60\%/20\%/20\% & 60\%/20\%/20\% & 50\%/25\%/25\% & 60\%/20\%/20\% & 60\%/20\%/20\% & 60\%/20\%/20\% &  \\
    $H_\text{agg}^{M}(G)$ & 0.8032 & 0.7768 & 0.694 & 0.6822 & 0.61  & 0.3566 & 0.5790 & 0.9904 & 0.9826 & 0.9432 &  \\
\midrule
    \midrule
          & \multicolumn{10}{c|}{Test Accuracy (\%) of State-of-the-art Models, Baseline GNN Models and ACM-GNN models} & Rank \\
    \midrule
    MLP-2 & 91.30 $\pm$ 0.70 & \underline{93.87 $\pm$ 3.33} & 92.26 $\pm$ 0.71 & 38.58 $\pm$ 0.25 & 46.72 $\pm$ 0.46 & 31.28 $\pm$ 0.27 & 66.55 $\pm$ 0.72 & 76.44 $\pm$ 0.30 & 76.25 $\pm$ 0.28 & 86.43 $\pm$ 0.13 & 23.40 \\
    \midrule
    GAT   & 76.00 $\pm$ 1.01 & 71.01 $\pm$ 4.66 & 78.87 $\pm$ 0.86 & 35.98 $\pm$ 0.23 & 63.9 $\pm$ 0.46 & 42.72 $\pm$ 0.33 & 61.09 $\pm$ 0.77 & 76.70 $\pm$ 0.42 & 67.20 $\pm$ 0.46 & 83.28 $\pm$ 0.12 & 26.20 \\
    APPNP & 91.80 $\pm$ 0.63 & 92.00 $\pm$ 3.59 & 91.18 $\pm$ 0.70 & 38.86 $\pm$ 0.24 & 51.91 $\pm$ 0.56 & 34.77 $\pm$ 0.34 & 67.21 $\pm$ 0.56 & 79.41 $\pm$ 0.38 & 68.59 $\pm$ 0.30 & 85.02 $\pm$ 0.09 & 22.80 \\
    GPRGNN & 91.36 $\pm$ 0.70 & 93.75 $\pm$ 2.37 & 92.92 $\pm$ 0.61 & 39.30 $\pm$ 0.27 & 67.48 $\pm$ 0.40 & 49.93 $\pm$ 0.53 & 66.90 $\pm$ 0.50 & 79.51$\pm$ 0.36 & 67.63 $\pm$ 0.38 & 85.07 $\pm$ 0.09 & 19.20 \\
    H2GCN & 86.23 $\pm$ 4.71 & 87.5 $\pm$ 1.77 & 85.90 $\pm$ 3.53 & 38.85 $\pm$ 1.17 & 52.30 $\pm$ 0.48 & 30.39 $\pm$ 1.22 & \underline{67.22 $\pm$ 0.90} & 87.52 $\pm$ 0.61 & 79.97 $\pm$ 0.69 & 87.78 $\pm$ 0.28 & 21.80 \\
    MixHop & 60.33 $\pm$ 28.53 & 77.25 $\pm$ 7.80 & 76.39 $\pm$ 7.66 & 33.13 $\pm$ 2.40 & 36.28 $\pm$ 10.22 & 24.55 $\pm$ 2.60 & 66.80 $\pm$ 0.58 & 65.65 $\pm$ 11.31 & 49.52 $\pm$ 13.35 & 87.04 $\pm$ 4.10 & 28.30 \\
    GCN+JK & 66.56 $\pm$ 13.82 & 62.50 $\pm$ 15.75 & 80.66 $\pm$ 1.91 & 32.72 $\pm$ 2.62 & 64.68 $\pm$ 2.85 & \underline{53.40 $\pm$ 1.90} & 60.99 $\pm$ 0.14 & 86.90 $\pm$ 1.51 & 73.77 $\pm$ 1.85 & \underline{90.09 $\pm$ 0.68} & 23.40 \\
     GAT+JK & 74.43 $\pm$ 10.24 & 69.50 $\pm$ 3.12 & 75.41 $\pm$ 7.18 & 35.41 $\pm$ 0.97 & 68.14 $\pm$ 1.18 & 52.28 $\pm$ 3.61 & 59.66 $\pm$ 0.92 & \underline{89.52 $\pm$ 0.43} & 74.49 $\pm$ 2.76 & 89.15 $\pm$ 0.87 & 20.90 \\
    FAGCN & 88.03 $\pm$ 5.6 & 89.75 $\pm$ 6.37 & 88.85 $\pm$ 4.39 & 31.59 $\pm$ 1.37 & 49.47 $\pm$ 2.84 & 42.24 $\pm$ 1.2 & 66.86 $\pm$ 0.53 & 88.85 $\pm$ 1.36 & \underline{\cellcolor[rgb]{ .816,  .808,  .808}\textbf{82.37 $\pm$ 1.46}} & 89.98 $\pm$ 0.54 & 18.20 \\
    BernNet & \underline{92.13 $\pm$ 1.64} & NA    & \underline{93.12 $\pm$ 0.65} & \underline{41.79 $\pm$ 1.01} & \underline{68.29 $\pm$ 1.58} & 51.35 $\pm$ 0.73 & NA    & 88.52 $\pm$ 0.95 & 80.09 $\pm$ 0.79 & 88.48 $\pm$ 0.41 & 14.75 \\
    GraphSAGE & 71.41 $\pm$ 1.24 & 64.85 $\pm$ 5.14 & 79.03 $\pm$ 1.20 & 36.37 $\pm$ 0.21 & 62.15 $\pm$ 0.42 & 41.26 $\pm$ 0.26 & OOM   & 86.58 $\pm$ 0.26 & 78.24 $\pm$ 0.30 & 86.85 $\pm$ 0.11 & 25.78 \\
    Geom-GCN* & 60.81 & 64.12 & 67.57 & 31.63 & 60.9  & 38.14 & NA    & 85.27 & 77.99 & 90.05 & 27.44 \\
    \midrule
    SGC-1 & 70.98 $\pm$ 8.39 & 70.38 $\pm$ 2.85 & 83.28 $\pm$ 5.43 & 25.26 $\pm$ 1.18 & 64.86 $\pm$ 1.81 & 47.62 $\pm$ 1.27 & 59.73 $\pm$ 0.12 & 85.12 $\pm$ 1.64 & 79.66 $\pm$ 0.75 & 85.5 $\pm$ 0.76 & 24.90 \\
    SGC-2 & 72.62 $\pm$ 9.92 & 74.75 $\pm$ 2.89 & 81.31 $\pm$ 3.3 & 28.81 $\pm$ 1.11 & 62.67 $\pm$ 2.41 & 41.25 $\pm$ 1.4 & 61.56 $\pm$ 0.51 & 85.48 $\pm$ 1.48 & 80.75 $\pm$ 1.15 & 85.36 $\pm$ 0.52 & 25.40 \\
    GCNII & 89.18 $\pm$ 3.96 & 83.25 $\pm$ 2.69 & 82.46 $\pm$ 4.58 & 40.82 $\pm$ 1.79 & 60.35 $\pm$ 2.7 & 38.81 $\pm$ 1.97 & 66.38 $\pm$ 0.45 & 88.98 $\pm$ 1.33 & 81.58 $\pm$ 1.3 & 89.8 $\pm$ 0.3 & 19.30 \\
    GCNII* & 90.49 $\pm$ 4.45 & 89.12 $\pm$ 3.06 & 88.52 $\pm$ 3.02 & 41.54 $\pm$ 0.99 & 62.8 $\pm$ 2.87 & 38.31 $\pm$ 1.3 & 66.42 $\pm$ 0.56 & 88.93 $\pm$ 1.37 & 81.83 $\pm$ 1.78 & 89.98 $\pm$ 0.52 & 16.40 \\
    GCN   & 82.46 $\pm$ 3.11 & 75.5 $\pm$ 2.92 & 83.11 $\pm$ 3.2 & 35.51 $\pm$ 0.99 & 64.18 $\pm$ 2.62 & 44.76 $\pm$ 1.39 & 62.23 $\pm$ 0.53 & 87.78 $\pm$ 0.96 & 81.39 $\pm$ 1.23 & 88.9 $\pm$ 0.32 & 20.90 \\
    Snowball-2 & 82.62 $\pm$ 2.34 & 74.88 $\pm$ 3.42 & 83.11 $\pm$ 3.2 & 35.97 $\pm$ 0.66 & 64.99 $\pm$ 2.39 & 47.88 $\pm$ 1.23 & OOM   & 88.64 $\pm$ 1.15 & 81.53 $\pm$ 1.71 & 89.04 $\pm$ 0.49 & 19.78 \\
    Snowball-3 & 82.95 $\pm$ 2.1 & 69.5 $\pm$ 5.01 & 83.11 $\pm$ 3.2 & 36.00 $\pm$ 1.36 & 65.49 $\pm$ 1.64 & 48.25 $\pm$ 0.94 & OOM   & 89.33 $\pm$ 1.3 & 80.93 $\pm$ 1.32 & 88.8 $\pm$ 0.82 & 19.11 \\
    \midrule
    ACM-SGC-1 & 93.77 $\pm$ 1.91 & 93.25 $\pm$ 2.92 & 93.61 $\pm$ 1.55 & 39.33 $\pm$ 1.25 & 63.68 $\pm$ 1.62 & 46.4 $\pm$ 1.13 & 66.67 $\pm$ 0.56 & 86.63 $\pm$ 1.13 & 80.96 $\pm$ 0.93 & 87.75 $\pm$ 0.88 & 17.00 \\
    ACM-SGC-2 & 93.77 $\pm$ 2.17 & 94.00 $\pm$ 2.61 & 93.44 $\pm$ 2.54 & 40.13 $\pm$ 1.21 & 60.48 $\pm$ 1.55 & 40.91 $\pm$ 1.39 & 66.53 $\pm$ 0.57 & 87.64 $\pm$ 0.99 & 80.93 $\pm$ 1.16 & 88.79 $\pm$ 0.5 & 17.70 \\
    ACM-GCNII & 92.62 $\pm$ 3.13 & 94.63 $\pm$ 2.96 & 92.46 $\pm$ 1.97 & 41.37 $\pm$ 1.37 & 58.73 $\pm$ 2.52 & 40.9 $\pm$ 1.58 & 66.39 $\pm$ 0.56 & 89.1 $\pm$ 1.61 & 82.28 $\pm$ 1.12 & 90.12 $\pm$ 0.4 & 14.30 \\
    ACM-GCNII* & 93.44 $\pm$ 2.74 & 94.37 $\pm$ 2.81 & 93.28 $\pm$ 2.79 & 41.27 $\pm$ 1.24 & 61.66 $\pm$ 2.29 & 38.32 $\pm$ 1.5 & 66.6 $\pm$ 0.57 & 89.00 $\pm$ 1.35 & 81.69 $\pm$ 1.25 & 90.18 $\pm$ 0.51 & 14.20 \\
    ACM-GCN & 94.75 $\pm$ 3.8 & 95.75 $\pm$ 2.03 & 94.92 $\pm$ 2.88 & 41.62 $\pm$ 1.15 & 69.04 $\pm$ 1.74 & 58.02 $\pm$ 1.86 & 67.01 $\pm$ 0.38 & 88.62 $\pm$ 1.22 & 81.68 $\pm$ 0.97 & 90.66 $\pm$ 0.47 & 7.90 \\
    ACM-GCN+ & 94.92 $\pm$ 2.79 & 96.5 $\pm$ 2.08 & 94.92 $\pm$ 2.79 & 41.79 $\pm$ 1.01 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{76.08 $\pm$ 2.13} & 69.26 $\pm$ 1.11 & 67.4 $\pm$ 0.44 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{89.75 $\pm$ 1.16} & 81.65 $\pm$ 1.48 & 90.46 $\pm$ 0.69 & 4.90 \\
    ACM-GCN++ & 93.93 $\pm$ 1.05 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{97.5 $\pm$ 1.25} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{96.56 $\pm$ 2} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{41.86 $\pm$ 1.48} & 75.23 $\pm$ 1.72 & 68.56 $\pm$ 1.33 & 67.3 $\pm$ 0.48 & 89.33 $\pm$ 0.81 & 81.83 $\pm$ 1.65 & 90.39 $\pm$ 0.33 & 4.30 \\
    ACM-Snowball-2 & 95.08 $\pm$ 3.11 & 96.38 $\pm$ 2.59 & 95.74 $\pm$ 2.22 & 41.4 $\pm$ 1.23 & 68.51 $\pm$ 1.7 & 55.97 $\pm$ 2.03 & OOM   & 88.83 $\pm$ 1.49 & 81.58 $\pm$ 1.23 & 90.81 $\pm$ 0.52 & 7.44 \\
    ACM-Snowball-3 & 94.26 $\pm$ 2.57 & 96.62 $\pm$ 1.86 & 94.75 $\pm$ 2.41 & 41.27 $\pm$ 0.8 & 68.4 $\pm$ 2.05 & 55.73 $\pm$ 2.39 & OOM   & 89.59 $\pm$ 1.58 & 81.32 $\pm$ 0.97 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{91.44 $\pm$ 0.59} & 7.22 \\
    \midrule
    ACMII-GCN & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{95.9 $\pm$ 1.83} & 96.62 $\pm$ 2.44 & 95.08 $\pm$ 2.07 & 41.84 $\pm$ 1.15 & 68.38 $\pm$ 1.36 & 54.53 $\pm$ 2.09 & 67.15 $\pm$ 0.41 & 89.00 $\pm$ 0.72 & 81.79 $\pm$ 0.95 & 90.74 $\pm$ 0.5 & 5.90 \\
    ACMII-Snowball-2 & 95.25 $\pm$ 1.55 & 96.63 $\pm$ 2.24 & 95.25 $\pm$ 1.55 & 41.1 $\pm$ 0.75 & 67.83 $\pm$ 2.63 & 53.48 $\pm$ 0.6 & OOM   & 88.95 $\pm$ 1.04 & 82.07 $\pm$ 1.04 & 90.56 $\pm$ 0.39 & 7.56 \\
    ACMII-Snowball-3 & 93.61 $\pm$ 2.79 & 97.00 $\pm$ 2.63 & 94.75 $\pm$ 3.09 & 40.31 $\pm$ 1.6 & 67.53 $\pm$ 2.83 & 52.31 $\pm$ 1.57 & OOM   & 89.36 $\pm$ 1.26 & 81.56 $\pm$ 1.15 & 91.31 $\pm$ 0.6 & 9.00 \\
    ACMII-GCN+ & 93.93 $\pm$ 3.03 & 96.75 $\pm$ 1.79 & 95.41 $\pm$ 2.82 & 41.5 $\pm$ 1.54 & 75.51 $\pm$ 1.58 & 69.81 $\pm$ 1.11 & 67.44 $\pm$ 0.31 & 89.18 $\pm$ 1.11 & 81.87 $\pm$ 1.38 & 90.96 $\pm$ 0.62 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{4.4} \\
    ACMII-GCN++ & 92.62 $\pm$ 2.57 & 97.13 $\pm$ 1.68 & 94.75 $\pm$ 2.91 & 41.66 $\pm$ 1.42 & 75.93 $\pm$ 1.71 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{69.98 $\pm$ 1.53} & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{67.5 $\pm$ 0.53} & 89.47 $\pm$ 1.08	 & 81.76 $\pm$ 1.25 & 90.63 $\pm$ 0.56 & 5.10 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
    \caption{Experimental results: average test accuracy $\pm$ standard deviation on $10$ real-world benchmark datasets. The best results are highlighted in grey and the best baseline results are underlined. Results "*" are reported from \cite{chien2021adaptive,lim2021new} and results "$^\dagger$" are from \cite{pei2020geom}. NA means the reported results are not available and OOM means out of memory. }
  \label{tab:acm.sota.random.split}%
\end{table}%


==> Tables1/gnn.vs.mlp.tex <==
% Table generated by Excel2LaTeX from sheet 'Results'
\begin{table}[htbp]
  \centering
  \small
  %\resizebox{\textwidth}{!}{
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|c|ccc|c}
    \toprule
    \toprule
    \multirow{2}[2]{*}{Datasets\textbackslash{}Models} & \multirow{2}[2]{*}{MLP} & \multirow{2}[2]{*}{GCN} & \multirow{2}[2]{*}{GAT} & \multirow{2}[2]{*}{GraphSAGE} & Baseline \\
          &       &       &       &       &  Average \\
    \midrule
    Cornell & 85.14 & 60.81 & 59.19 & 82.97 & 67.66 \\
    Wisconsin & 87.25 & 63.73 & 60.78 & 87.84 & 70.78 \\
    Texas & 84.59 & 61.62 & 59.73 & 82.43 & 67.93 \\
    Film  & 36.08 & 30.98 & 29.71 & 35.28 & 31.99 \\
    Chameleon & 46.21 & 61.34 & 61.95 & 47.32 & 56.87 \\
    Squirrel & 29.39 & 41.86 & 43.88 & 30.16 & 38.63 \\
    Cora  & 74.81 & 87.32 & 88.07 & 85.98 & 87.12 \\
    Citeseer & 73.45 & 76.70 & 76.42 & 77.07 & 76.73 \\
    Pubmed & 87.86 & 88.24 & 87.81 & 88.59 & 88.21 \\
    DBLP  & 77.39 & 85.87 & 85.67 & 81.19 & 84.24 \\
     Coauthor CS & 93.72 & 93.91 & 93.41 & 94.38 & 93.90 \\
     Coauthor Phy & 95.77 & 96.84 & 96.32 & OOM   & 96.58 \\
     AMZ Comp & 83.89 & 87.03 & 89.44 & 83.70 & 86.72 \\
    AMZ Photo  & 90.87 & 93.61 & 94.12 & 87.97 & 91.90 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    %}
    \caption{Accuracy (\%) Comparison of Baseline GNNs and MLP }
  \label{tab:gnn.vs.mlp}%
\end{table}%

%\small
%\setlength{\tabcolsep}{3pt}
%\iffalse \caption{Comparison of Baseline GNN Models and MLP}
%\label{tab:comparison_baselines_mlp}%
%\if
